Mobile Microphone Array Speech Detection and Localization in Diverse Everyday Environments

Joint sound event localization and detection (SELD) is an integral part of developing context awareness into communication interfaces of mobile robots, smartphones, and home assistants. For example, an automatic audio focus for video capture on a mobile phone requires robust detection of relevant acoustic events around the device and their direction. Existing SELD approaches have been evaluated using material produced in controlled indoor environments, or the audio is simulated by mixing isolated sounds to different spatial locations. This paper studies SELD of speech in diverse everyday environments, where the audio corresponds to typical usage scenarios of handheld mobile devices. In order to allow weighting the relative importance of localization vs. detection, we will propose a two-stage hierarchical system, where the first stage is to detect the target events, and the second stage is to localize them. The proposed method utilizes convolutional recurrent neural network (CRNN) and is evaluated on a database of manually annotated microphone array recordings from various acoustic conditions. The array is embedded in a contemporary mobile phone form factor. The obtained results show good speech detection and localization accuracy of the proposed method in contrast to a non-hierarchical flat classification model.

==> Two-Stage-Hierachical (arxiv)/abstract.tex <==
Joint sound event localization and detection (SELD) is an integral part of developing context awareness into communication interfaces of mobile robots, smartphones, and home assistants. For example, an automatic audio focus for video capture on a mobile phone requires robust detection of relevant acoustic events around the device and their direction.
Existing SELD approaches have been evaluated using material produced in controlled indoor environments, or the audio is simulated by mixing isolated sounds to different spatial locations.  
This paper studies SELD of speech in diverse everyday environments, where the audio corresponds to typical usage scenarios of handheld mobile devices. In order to allow weighting the relative importance of localization vs. detection, we will propose a two-stage hierarchical system, where the first stage is to detect the target events, and the second stage is to localize them. 



The proposed method utilizes convolutional recurrent neural network (CRNN) and is evaluated on a database of manually annotated microphone array recordings from various acoustic conditions. The array is embedded in a contemporary mobile phone form factor. The obtained results show good speech detection and localization accuracy of the proposed method in contrast to a non-hierarchical flat classification model.

% THIS MIDDLE PARAGRAPH WAS REMOVED BY PASI 
% At the first stage, the sound event classification utilizes magnitude spectrum features and their temporal sequence within a convolutional recurrent neural network (CRNN). At the second stage, each speech sequence is classified with regard to whether it arrives from the front and/or back direction of the array. This  direction estimation uses spatial features between microphone signals as input to a second CRNN. 




%Results show good speech detection and localization accuracy with a collected multi-microphone audio  database, consisting of material from various acoustic conditions. %The used mobile array consisted of eight microphones embedded in a smartphone form factor. %We then manually annotated the sound event type, and when present the speaker directions, with one-second temporal resolution. Several event labels within a one-second block were allowed. 

%

%Secondly, the time resolution for classification can be instantaneous or over a time-period. While this largely depends on the application, time-periods attached with multiple labels of events occurring within the period consume less time for manual annotation than exact labels. %* \textit{AE: the previous sentence is unclear: is it trying to say that we propose a method of speeding up annotation work by dividing data into one-second chunks and then annotating all the labels within a chunk? Or what is the main point?}
 
%\textit{AE: abstract is a bit weak, needs improvement. Clearly state the main content/results of the paper, why would someone want to read the paper? Now main results are missing completely.}
 
% Producing annotations with precise time and direction annotations for different types of sound event from real life recordings can be prohibitive due to costs. To mitigate this issue, annotations were made for longer blocks of audio with multiple labels and only the direction of a speakers were annotated. 
 
%Such annotations pose a challenge for the automatic detection and localization design, which is here proposed to be solved with a two-stage hierarchical approach. The first stage recognizes the sound class, and passes it to the direction classifier if it was detected as speech. The collected database consists of one second blocks of labeled audio from different types of indoor and outdoor environments, collected with an eight channel microphone array embedded in a smartphone form factor. 

==> Two-Stage-Hierachical (arxiv)/baseline.tex <==
\ssubsection{Baseline}\label{sec:baseline}
The baseline comparison method is a flat CRNN classifier with three binary labels for each of the classes. The spatial features described in Section~\ref{sec:localization} are   only used, since i) the magnitude spectrum features could not be concatenated to spatial features due to the different frame lengths, and ii) the used spatial features already contain magnitude spectrum difference information. A similar training process as in Section~\ref{subsec:speechtrain} is used, but instead of speech-only F1-score, the weighted average F1-score over all three labels is used as the early stopping criteria. 
 The best model had 360k parameters.
%To prevent this, the error resulting from the class samples is weighted with the inverse value of their relative amount. As a result the samples in the "Both" class contribute an equal amount to the objective functions as the other two classes. The weighting value was empirically raised to the power 1.5 to further emphasize the effect. 



==> Two-Stage-Hierachical (arxiv)/dataset.tex <==


\input tabledata.tex

%\subsection{Data collection and annotation}
\paragraph*{Data collection and annotation}

%\hl{Aapo, your role is to briefly describe the recording setup (device setup (cameras, mics), data rate, annotation accuracy) for the real data only.


%You can use figures, but I’d limit them to two figures side-by-side. Maybe a picture of the recording device, and then an example picture of a video where providing a feel for the data. Data statistics, how many seconds of data we have in different environments.}

 Acoustic data for training and evaluation of the methods was collected in complex real-life environments. Actions and objects in the recordings aim to represent typical contents of casual videos recorded by a typical mobile phone user. The data set contains speech and other scene-specific sounds from common scenarios such as sports, moving vehicles and live music. In total there are 24 environment types including both indoor- and outdoor scenes, refer to Table~\ref{tab:environments}. %The environment types used in the recordings and the amounts of data (in 1-second blocks) for each environment are listed in Table~\ref{tab:environments}.
 The duration of the recordings varies from 10 to 180 seconds, and the total duration is 89~min. % duration of recorded audio data is 89~minutes.
 
 
% Three recording devices were used in the data collection.
The audio data was collected with an eight-channel microphone array mounted to a custom 3D-printed rigid phone-shaped body. In addition, a 360$^\circ{}$ camera was used to make the annotation task easier and a web camera was used to collect video material for later research purposes. The devices were fixed to a hand-held microphone stand during the recordings that was was held from a grip below to prevent obstructing sensors. %the effect of microphones being covered by fingers.
  %
 Figure~\ref{fig:arraypictures} illustrates the recording setup and the microphone array. 
 %
 %Refer to Fig.~\ref{fig:arraypic} for pictures of the recording setup, and Fig.~\ref{fig:array} for the microphone array.
 A laptop was used to collect the eight-channel audio as wav files at 48~kHz sampling rate and 32-bit resolution. 
%  The recording of the microphone array was controlled with a laptop and the audio files produced are in eight-channel wav-format with a sampling rate of 48 kHz and resolution of 32-bits.  %The placement of the microphones is illustrated in Fig.~\ref{fig:array}.

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=.4\columnwidth,trim = {0mm 0mm 0mm 0mm}, clip]{arraypic.jpg}\vspace{-2mm}
%    \caption{Pictures of the microphone array and other accompanying devices.}
%    \label{fig:arraypic}
%    \vspace{-5mm}
%\end{figure}




The recorded signals were annotated with the following labels using one-second resolution: % The classes used in the annotations are %(1) A person holding the microphone array is speaking, (2) Other people near the array are speaking 
%  \begin{enumerate}[wide, labelwidth=!, labelindent=0pt,nosep, label={(\arabic*)}]
 (1)~{\bf Speech back}: A person was speaking from behind the microphone array, e.g., the person holding the device. 
(2)~{\bf Speech front}: A person in  front of the array was speaking.  
(3)~{\bf Something else}: An object was emitting interesting non-speech sound.
%\end{enumerate}
Multiple labels were allowed to be used simultaneously. The direction for the class "something else" was not used, since it was not considered as interesting as for the speech. Besides, the direction for this class is often ambiguous and rather hard to annotate.
%If no labels were assigned, the block was considered as background noise.

A sound was considered interesting if the sound source was  the focus of the recording or the sound was otherwise special in the context of the environment. For example, a scenario on a beach where a diver jumped into water in front of the array was assigned the label "Something else" during the time of a splash. Other swimmers talking in the background and creating similar splashing sounds were considered as background, since they were not in a key role from the perspective of the cameraman. Therefore, the boundary between interesting sounds and background noise is inevitably ambiguous, since the same sound can be assigned a label or considered as background noise depending on the situation. A general guideline used in the annotations was that when a sound source was close to the array and the sound was audible inside a block of data, it was assigned with the corresponding label. Other examples of  sounds labeled "Something else" include a guitar, a racing car, and a table tennis ball. All speech related sounds such as singing and whispering were assigned with labels "Speech back" and/or "Speech front". Multiple labels were assigned when multiple sound sources were present inside the one-second clip, including multiple sound sources of the same type. Audio blocks where a speech source is in the left or right directions % $\pm 30^\circ{}$
were omitted   due to ambiguous front/back direction. %Multiple classes can be active at the same time, including multiple sound sources of the same class.

%Directions of the annotated speech sounds were also labeled for each block of data. The directions used are front and back, determined by the location of the sound source with respect to the microphone array. 





%\begin{figure}[t]
%    \centering
%    \includegraphics[width=.6\columnwidth,trim = {50mm 22mm 35mm 33mm}, clip]{frontback.png}\vspace{-2mm}
%    \caption{An illustration of the eight microphone placements and the directions "Front" and "Back" used to annotate the speaker direction. The x,y,z dimensions of the devices are: 140, 65, and 7~mm.}
%    \label{fig:array}\vspace{-2mm}
%\end{figure}


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.4\columnwidth}
     \includegraphics[width=\columnwidth,trim = {0mm 0mm 0mm 0mm}, clip]{arraypic.jpg}\vspace{-2mm}
     \caption{Pictures of the microphone array and other accompanying devices.\label{fig:arraypic}}
     
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.55\columnwidth}
      \centering
    \includegraphics[width=\columnwidth,trim = {50mm 22mm 35mm 33mm}, clip]{frontback.png}\vspace{-2mm}
    \caption{An illustration of the eight microphone placements and the directions "Front" and "Back" used to annotate the speaker direction. The x,y,z dimensions of the devices are: 140, 65, and 7~mm.\label{fig:array}}
    \end{subfigure}
\caption{Recording setup~(a), and microphone layout~(b).\label{fig:arraypictures}}
\vspace{-6mm}
\end{figure}

%\ssubsection{
\paragraph*{Database for machine learning}
The audio was divided into six different folds. For the first five folds, the data was distributed so that each fold had the same proportion of \mbox{1-s} blocks captured in an inside and outside environment as the whole data set. Each recording was used as a whole in a single fold, and no recording was split between several folds. The sixth fold %was added later to include more
includes most data from speech sources simultaneously in front and back. 
Table~\ref{tab:classdir} displays the amount of \mbox{1-s}~blocks per each label class. It also includes counts for the cases where speech is present either back or front, and also back \emph{and} front.
%For blocks labeled to contain speech, the number of blocks  with speech only in front, speech only in back, and speech in both directions is listed separately. 

%The first column is the fold index, the second and third columns show the number of frames with the label "something else" and "speech" correspondingly, followed by a column with the total number of annotated frames. The rightmost three columns show the amount of samples in the different location categories. 

%
%\hl{Eemi, your role is the descibe the data statistiscs, how much data in different environments we have, how data is split into folds. 

%You can use table to compactly represent the relevant statistics.  Make the table 1 column wide, and use as few rows as possible. The default table can be heavily squeezed, so don't worry if it is too wide in the beginning. (we can remove padding, and reduce fonts).
%}
%Initial data was divided into five folds for cross-validation.




%Fold 1: 871 frames, out of which: 376 include: Speech label  (43.17 %), Else label: 376. 	 FO: 187,	 BO: 177,	 F&B: 12, silence: 213
%Fold 2: 748 frames, out of which: 310 include: Speech label  (41.44 %), Else label: 292. 	 FO: 61,	 BO: 243,	 F&B: 6, silence: 218
%Fold 3: 768 frames, out of which: 383 include: Speech label  (49.87 %), Else label: 187. 	 FO: 98,	 BO: 271,	 F&B: 14, silence: 305
%Fold 4: 892 frames, out of which: 407 include: Speech label  (45.63 %), Else label: 327. 	 FO: 173,	 BO: 204,	 F&B: 30, silence: 327
%Fold 5: 719 frames, out of which: 201 include: Speech label  (27.96 %), Else label: 357. 	 FO: 24,	 BO: 176,	 F&B: 1, silence: 307
%Fold 6: 1025 frames, out of which: 967 include: Speech label  (94.34 %), Else label: 0. 	 FO: 291,	 BO: 576,	 F&B: 100, silence: 58



\addtolength{\tabcolsep}{-4pt} 

\begin{table}[b]\vspace{-3mm}
    \centering
        \caption{Label appearance statistics for the folds. Note that any combination of labels can be present during a single block.}\vspace{-2.3mm}
    \label{tab:classdir}
    \scalebox{.87}{
    \begin{tabular}{c|c||c|c|c| |c|c|c }
    \toprule
   Fold & Total & Something & Speech Front  &  No & %\multicolumn{3}{c}{Direction classes for speech labels}
   Speech & Speech & Speech Front \\
     \#             & blocks & Else & or Back  &  labels &  Front only &  Back only &   and Back  \\
    \toprule
    
    
    1               & 871   & 376 & 376 & 213   &  187     & 177 & 12     \\
     
    2             & 748    &  327 & 310 & 218    &  61 & 243 & 6      \\
    
    3               & 768   & 187 & 383 & 305   &  98     &  271 & 14     \\
    
    4              & 892  & 292 &  407  & 327    &  173     & 204 & 30      \\
     
    5              & 719  & 376 &  201 & 307    &  24     &  176   & 1  \\
     
    6              & 1025  & 0 & 967 & 58    &  291     & 576 & 100      \\
    \end{tabular}
    } 

\end{table}
\addtolength{\tabcolsep}{4pt} 


==> Two-Stage-Hierachical (arxiv)/detection.tex <==
In the sound classification stage, given a \mbox{1-s} block of audio, the aim is to recognize if there is speech and/or any other interesting sound events (\textit{i.e.} "something else" class) present at any time. The output of this stage is a probability value for both of these labels. Sound classification is done by feeding time-frequency acoustic features extracted from audio to a deep neural network that estimates the class probabilities. Feature extraction and classification are elaborated below.

%In the first step, time-frequency domain acoustic features are extracted from the audio. In the second stage, a \ac{DNN} maps the features into class probabilities. %based model is trained to do classification using the acoustic features as input, and the manually obtained sound annotations as target output. 


\begin{figure}[t]
    \centering
    \includegraphics[width=0.67\linewidth]{figs/detection/framework.eps}\vspace{-1mm}
    \caption{Joint classifier system framework for detection and localization of sound events. First stage detects the type of sound, second stage  estimates direction of detected speech.}
    \label{fig:framework}\vspace{-5mm}
\end{figure}

\ssection{Acoustic Feature Extraction}
\label{subsec:clsf_feat_ext}
%In the acoustic feature extraction stage, the given multi-channel audio is first combined, then log mel spectrogram is calculated and finally, the features are scaled in order to be fed to the DNN as input. 
%The feature extraction pipeline is presented in Figure~\ref{fig:feature_extraction}.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\linewidth]{figs/classification/feature_extraction.eps}
%     \caption{Acoustic feature extraction pipeline for the sound event classification. The output shapes at several steps of the pipeline are given in brackets.}
%     \label{fig:feature_extraction}
% \end{figure}

%\paragraph*{Pre-processing step}
In a pre-processing step, the multi-channel audio is converted to mono by taking the average over the channels at each sample. The resulting monophonic audio signal is amplitude normalized by dividing with the maximum absolute value. % in the given one-second audio block. %The assumption for using monophonic audio is that the direction information, which can possibly be extracted from the channel differences, is  irrelevant to the sound classification. % In other words, we are rather interested in the content and not the direction of the sound. Nevertheless, experiments using multi-channel audio features have been conducted an reported in Section~\ref{sec:speechres}.


\paragraph*{Log-Mel Spectrogram Estimation}
The log-mel spectrogram features were obtained using 20 ms frames and 10 ms overlap in 40 mel frequency bands. The features are standardized to zero mean and unity variance using statistics from the training set.

% agnitude spectrogram is estimated using the \ac{STFT} with 20 ms frames and 10 ms overlap, and
%In order to estimate the log mel spectrogram, the magnitude spectrogram for each frame is multiplied by the coefficients of a 40-band mel filterbank. Then, a logarithm operation with added value of 0.001 (for stability) is applied. %\textit{AE: would appreciate some comments/references on why we still use traditional feature extraction and not let the network learn the features?}


%\paragraph*{Magnitude Spectrogram Estimation}
%The magnitude spectrogram is estimated by first dividing the audio into short, 20 ms frames with 10 ms overlap (to satisfy the stationary sinusoid assumption of the Fourier transform), multiplying each frame with a Hann window (to avoid boundary discontinuity problems), taking the discrete Fourier transform (DFT), and finally converting the resulting complex values into real by taking the magnitude and obtaining the magnitude spectrogram. 

%\paragraph*{Log Mel Spectrogram Estimation}
%In order to estimate the log mel spectrogram, the magnitude spectrogram for each frame is multiplied by the coefficients of a 40-band mel filterbank. Then, logarithm operation with a stabilizer of 0.001 is applied.

%\paragraph*{Scaling}
%The \ac{DNN} weights are often initialized with random values close to zero. Having consistently very large (or very small) values as \ac{DNN} input would affect the neuron outputs and loss gradients, resulting with a slower learning. Therefore, in order to reach a minimum in the loss curve faster, the obtained acoustic features (log mel spectrogram) are scaled to zero mean and unit variance at each mel band. The scaling parameters are obtained from the collective one-second blocks of the training set, and the same parameters are applied also on the validation and test sets.

\ssection{Deep Neural Network Model}\label{subsec:speechtrain}

The DNN technique utilized in the sound classification is a \ac{CRNN}. % CRNNs have theoretical advantages for sound classification in real-life environments, where sound events may exhibit wide variations in their frequency content and temporal structure.
Convolutional layers use small, shifting 2D kernels to extract higher level features that are invariant to local spectral and temporal variations. Recurrent layers are effective in modeling the longer term temporal context for the sound events. Combining convolutional and recurrent layers has been found suitable for various audio classification tasks such as sound event classification~\cite{cakir2017convolutional}, automatic speech recognition~\cite{amodei2016deep} and music genre classification~\cite{choi2016convolutional}.

The details of the CRNN architecture are as follows. Each 5-by-5 convolutional layer is followed by a rectified linear unit (ReLU) activation, and max-pooling by two in both time and frequency dimensions. The 3D output of the final convolutional layer is converted into 2D by reshaping the frequency and channel dimensions into a single dimension. This output is fed to one or multiple recurrent layers (long-short term memory~(LSTM)~\cite{hochreiter1997long} layers specifically). The LSTM output is fed to a fully connected feed-forward layer with logistic sigmoid activation that applies the same weights over each time step of the input. The resulting output at each time step are the two label probabilities of the i) speech presence using the merged "Speech Front" and "Speech Back" labels, and ii) "Something Else". Finally, max-pooling over time is applied over the sequence, and the two label probabilities are obtained for the one-second block of audio. The binary label predictions are obtained by using a threshold value of $0.5$ for the output probabilities.  

%The network training procedure is as follows. 
The network is trained to minimize the cross-entropy between the estimate output and the target output. Adam~\cite{Kingma:ICLR:2015} is used as the optimizer. After each epoch, the F1-score for the merged "speech" labels for the validation set is calculated. % If it is better than the best one from the earlier epochs, the model at that epoch is saved. 
 If the model does not improve for 25 epochs, the training is terminated. The best model based on the validation set score is used for testing.  In total, 197 different hyper-parameter combinations were evaluated with different amounts and configurations of the convolutional layers and the recurrent layers. The best model had 611k learnable parameters.



==> Two-Stage-Hierachical (arxiv)/introduction.tex <==

Sound source localization (SSL) aims to determine either the direction or position of the source in a continuous or discrete-valued space, and automatic sound event detection (SED) aims to recognize the classes of the source sounds present, and estimate their temporal activities.  
%to produce a symbolic description of detected sounds in the analyzed content.
 The SSL and SED have been extensively researched mostly as separate problems. Deep learning methods have brought improvements in SSL performance \cite{Xiao:ICASSP:2015,Chakrabarty:WASPAA:2017,Yalta:JRM:2017,Adavanne:EUSIPCO:2018, Vera-Diaz:MDPI:2018,Salvati:2018,VESPERINI201883,Pertila:2017:ICASSP,pertila:ICASSP:2019,Wang2018} and in SED~\cite{piczak2015environmental,takahashi2016deep,salamon2017deep,cakir2017convolutional} over traditional approaches. Recent approaches solving simultaneously the SED and SSL problems, i.e., joint sound event detection and localization (SELD) problem, include using \acp{CNN}~\cite{hirvonen2015classification,He2018:IS},   \ac{CRNN}~\cite{adavanne2018sound,cao2019polyphonic, politis2020overview}, and the Least Absolute Shrinkage and Selection Operator (LASSO)~\cite{8928942}. 
 % The best structure of SELD network is an open research question and weight transfer from a CNN or CRNN SED network to a similarly structured SSL network has been proposed~\cite{}. The work in~\cite{8928942} relies on Least Absolute Shrinkage and Selection Operator (LASSO) approach for binaural SELD instead of deep learning. 

As the research in the field has progressed towards machine learning approaches, the data used to train a system has a crucial impact on its performance. Larger and more diverse datasets enable learning more complex models that will generalize better to new conditions.
%A system can be expected to work well with data that is similar to the one that has been used for training. A large mismatch between training and testing data typically leads to significant drop in performance.
Since recording of acoustic scenes with spatiotemporal annotations is an extremely difficult task, there are no large-scale datasets of real scenes, and existing smaller ones are limited to evaluation of algorithms and are unsuitable for training deep-learning methods (e.g. LOCATA challenge \cite{evers2020locata}). That is in contrast, e.g., to automatic speech recognition where annotation is not a problem and recorded datasets exist with diverse range of conditions (e.g., the ASpIRE \cite{harper2015automatic} and CHiME \cite{barker2018fifth} challenges). Hence, for deep-learning based SSL researchers have generally relied on either simulations for training and testing on a small recorded dataset \cite{perotin2019crnn, nguyen2020robust}, or on emulated scenes with real recorded room impulse responses (RIRs). The second option allows integrating real acoustics with source signals of interest with a few RIR datasets available \cite{hadad2014multichannel, jeub2009binaural, stewart2010database}. Additionally, the SELD datasets related to the DCASE challenge have been generated with a large scale RIR collection from 15 rooms and a spherical microphone array \cite{politis2020overview}. The only annotated dataset for SELD with real recordings we are aware of is the one in \cite{brousmiche2020secl} for office environments.


 In this study, a microphone array embedded inside a flat mobile phone body was used to collect a dataset from diverse everyday environments to obtain insights for realistic mobile phone applications of the SELD approaches. To our knowledge, a microphone array in a mobile phone form factor has not been dealt with in previous SELD research. The flat microphone array shape imposes challenges to the spatial resolution rendering the task more difficult in contrast to, e.g., spherical arrays. Therefore, we do localization using only two categories, \emph{front} and \emph{back}, with respect to a mobile phone screen. This is motivated by possible mobile phone multimedia applications. % such as using the proposed method as a trigger for automatic audio focus emphasizing relevant sounds from a certain direction.
  We focus the evaluation on localization and detection of speech % because  of its importance in most applications,
  and detection of other prominent sounds of interest without localizing them.
 


%The time labeling resolution for detection and localization can be accurate (strong) or over a time-period (weak). The strong labeling demands high temporal resolution in both the spatial location and in the sound class annotations, which requires significant manual work. In contrast, providing weak labels of sound locations and classes reduces the annotation work at the cost of temporal resolution, which is also referred as tagging~\cite[Ch.~6]{virtanen2018computational}. However, the corresponding detection task becomes more difficult. While research for SED has dealt  with weak labels~\cite{adavanne2017sound}, the previous state-of-the-art SELD has relied on strong labels only and synthetic sound scenes providing those labels.

%In this work, the goal is to classify the direction of detected speech sources using weak labels for time-periods of one second, referred as a block, to retaining a moderate temporal resolution.  Location information from the other classes is omitted, which reduces the time required to annotate real-life databases that are needed for the development of the methods. For this aim, a two-stage hierarchical classification approach is proposed to first detect the speech class presence and then to provide a direction for any detected speech.


%SELD approaches inherently place equal importance for both the type of detected sound and its location. % For example, in the case of speech and interference classification and localization, the approach can require directional reference information from interference and speech sources~\cite{He2018:IS}. 
%
%
 %detected sounds by limiting the localization to the most relevant detected classes. 
 %
%
State of the art SELD systems typically train a single system for joint localization and detection. In order to allow controlling the relative importance of localization vs. detection, we  propose a hierarchical approach of two separate deep neural networks, optimized for their corresponding tasks. %The detection part assigns "speech" and "something else" labels to each one second block. The localization network assigns a direction label "front" and "back" to each frame detected as speech.

%T  into two application motivated categories: {\emph front}, and \emph{back} with respect to a mobile phone screen
 %
 % 
 %The motivation is to reduce the annotation work while retaining a moderate temporal resolution.  

 %
%To investigate the proposed approach, a database was recorded and annotated with a time resolution of one second, referred as a block. This relaxed time resolution further reduces the cost of manual annotation, since each block is assigned multiple labels without more detailed timing information, also referred as tagging or weak labeling~\cite[Ch.~6]{virtanen2018computational}.However, the uncertainly of sound occurrence and location is limited to one second. % Each block is annotated with labels speech front, speech back, and {\it{else}} for anything non-speech other than background, i.e. interesting sound events such as music, horns, etc.   
 %
 %


%This paper describes the database collection, presents the sound source dependent weak labeling approach, addresses the SELD problem by a novel hierarchical two-stage deep neural network approach, and then compares the results to a baseline classifier.

In this paper Section~\ref{sec:data} describes the database collection. % setup and presents the sound source dependent weak labeling approach. 
Section~\ref{sec:method} describes the proposed hierarchical two-stage SELD approach. Section~\ref{sec:results} describes the evaluation of the SED, SSL, and the joint system and then compares the results to a baseline classifier. Finally,  Section~\ref{sec:conclusions} draws the conclusions and future directions. 


==> Two-Stage-Hierachical (arxiv)/locred.tex <==

%
%
Table~\ref{table:resdir} depicts the confusion matrix for the different location classes during frames with annotated speech. The results are obtained by accumulating the binary test folds label predictions over the six folds (i.e. k-fold cross-validation). The direction classifier is described in Section~\ref{sec:localization}. 
 %
%Based on a grid search, the best network parameters were
%a CNN kernel size of $3\times3$ with 32 feature maps, 
%128 neurons in the fully connected layers, 
%an $\ell_2$-regularization value of 0.01 in the CNN and fully connected layers, and 
%a dropout probability $p=0.25$ before the output layer. The adagrad optimizer and a mini-batch size of 64 samples were used.  
%
%
 The speech emitted from the back direction was more accurately recognized than speech from the front. This is expected, since all the samples of a speaker holding the device are labeled with "Speech back". Since they were emitted close to the array, they inherently had a better SNR in contrast to the front direction, which contained more distant talkers. The cases where both the directions were active are detected with the least accuracy. This can be attributed to having the least amount (only 6~\%) of data from such cases. 

%\textit{AE: also here, please consider presenting overall results first and then confusion matrices}
%Macro and micro averaged F1-scores are 0.676 and 0.911 respectively.

%peech front precision, recall, F1 score at thr 0.5: 0.9184, 0.9478, 0.9329
%peech back precision, recall, F1 score at thr 0.5: 0.9165, 0.9519, 0.9339
%inal F1 score = 0.933519202229. (Average over both labels)
%onfusion matrix, without normalization
%[   0    0    0    0]
%[   0  676   20  138]
%[   0   23 1558   66]
%[   0   58   28   77]]
%ormalized confusion matrix
%[       nan        nan        nan        nan]
%[0.         0.81055156 0.02398082 0.16546763]
%[0.         0.01396478 0.94596236 0.04007286]
%[0.         0.35582822 0.17177914 0.47239264]]







%%%%%%%%% baeline 





\fi




==> Two-Stage-Hierachical (arxiv)/results_detection.tex <==
% TABLE MOVED BEFORE 
% results for the speech and something else classification
% This section describes the classification results for the speech detection.

%\ssection{Overall performance}





%\begin{figure}
%    \centering
%    \includegraphics[width=0.6\linewidth]{figs/detection/test_311_fold_avg.png}
%    \caption{Confusion matrix of the proposed CRNN method. The instances where both %classes are present are treated as a separate class for the visualization.}
%    \label{fig:clsf_overall}
%\end{figure}





%The overall performance of the proposed \ac{CRNN} method for sound classification is presented in Table~\ref{table:clsf_overall}. 
The confusion matrix for the two-stage \ac{CRNN} speech classification model is given in Table~\ref{fig:clsf_overall} and the baseline results for comparison with speech direction outputs merged into a single class are given in  Table~\ref{fig:clsf_overall_baseline}. The instances where both classes are present are treated as a separate class for the visualization. The sample numbers inside each box are obtained by % binarizing the test set predictions with the threshold 0.5, and
 accumulating the binary output of the test fold values of the six folds using  k-fold cross-validation. %\textit{AE: why present confusion matrix first and only then overall results? Would first present overall results, then go deeper into confusion matrix and probably explain a bit about the confusions.}
 The percentage values represent the fraction of the predicted labels assigned for each audio block with the corresponding true label. 
 
 The hierarchical approach has better classification performance in almost all classes ("Silence", "Speech", "Both") except for the "Else"  class in contrast to the baseline. 
 
%The informal listening tests and output visualizations point to the fact that a significant amount of the errors for classifying speech happen around the onset and offset points. These are often ambiguous regions where it is quite hard even for humans to pinpoint the exact onset and offset points. In addition, the 

The "Something else" performance is quite low in both approaches compared to the class "Speech". This can be attributed to i) the labeling ambiguity problem, and ii)  to the scarcity of data, which makes it hard to capture the characteristics of all the various types of sound events that are included in this class.  



%(see \textit{e.g.} Figure~\ref{fig:sed_vis_example} in Section~\ref{sec:jointres})





% \subsubsection{Performance vs. SNR}

% The performance of the speech classifier vs. SNR is presented in Figure~\ref{fig:acc_vs_snr_267}. The simulated data creation procedure is explained in Section~\ref{sec:simulation}. For these experiments, since the simulated data does not include the \textit{else} class examples, the CRNN model provides the presence probabilities only for the speech class. 

% Apart from fold 3, the F1 score decreases sharply after around -9 dB SNR. It should be noted that for fold 3, it was noticed that one of the three background samples used in this fold had inconsistent energy level distribution in time, which affected the SNR measurement and resulted with a less challenging setup in some portions of the recording. Since it is hard to prove the level of difficulty for these simulated recordings through SNR values, the reader is kindly encouraged to listen to these recordings provided as deliverables. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\linewidth]{figs/detection/acc_vs_snr_267.eps}
%     \caption{F1 score vs. SNR using only simulated data. In training, data from all SNR levels are used. During testing, data from each SNR level is evaluated separately.}
%     \label{fig:acc_vs_snr_267}
% \end{figure}

%\ssection{Effect of multi-channel feature extraction}
%The log mel spectrogram feature extraction method explained in Section~\ref{subsec:clsf_feat_ext} (labeled as \textit{average\_time}) used time-averaging of the microphone signals to obtain the monophonic signal from which the features were extracted. There are also other methods of how the multi-channel properties of audio can be utilized in the feature extraction for sound classification. One way is to calculate the log mel spectrogram features for each channel, and then combine them to form a 3D input for the first convolutional layer of the \ac{CRNN} (labeled as \textit{multi}). Another way is to simply calculate the features using only the first channel (labeled as \textit{first}). Finally, one can calculate the mel band \textit{multi} features, take the average over the channels and finally take the logarithm to obtain the average log mel band spectrogram (labeled as \textit{average\_mel}). The performance for each of these methods is given in Table~\ref{table:multifeat}. It can be concluded that there is not a significant benefit in utilizing the direction information present in the multi-channel audio for better speech classification.%, and the initially implemented feature extraction method (converting the signal to mono in raw audio domain) performs the best for speech.
%\arrayrulecolor{black} %Table line colors

%\begin{table}[b]
%    \centering\vspace{-5mm}
%        \caption{Speech F1 score vs. mel feature extraction method.}
%    \label{table:multifeat}
%    \scalebox{1}{
%    \begin{tabular}{c|c|c}
%    F1 & Speech & Else \\
%    \toprule
%        First & 83.4 & 64.0 \\
%        Multi &  85.6 & 62.8\\
%        Average\_mel & 86.3 & \textbf{64.7}\\
%        Average\_time & \textbf{87.0} & 63.0
%    \end{tabular}}
%
%\end{table}

%\ssection{Model ensemble}
%
%An effective method to improve the DNN performance is to average the probability outputs of several independently trained models. This helps to filter the noise in individual models. The models to be used in the ensemble is selected from the models that perform the best over the grid search experiments. 

%The results comparing the best performing model and the ensemble of top-4 models are presented in Table~\ref{table:ensemble}.
%\begin{table}
%    \centering
%    \begin{tabular}{c|c|c}
%    F1 & Speech & Else \\
%    \toprule
%        Single &  88.4 & 69.7\\
%        Ensemble & 89.5 & 69.2 \\
%    \end{tabular}
%    \caption{Single model vs. model ensemble.}
%    \label{table:ensemble}
%\end{table}

%\ssection{Performance vs. binarizing threshold}
%For the classification of sound events, F1 score is one of the most commonly used metrics and it is often evaluated with the unbiased threshold of 0.5. On the other hand, for the real-life implementation of such a system, it may be desired to adjust the threshold depending on the application preferences (higher precision, higher recall etc.). 

%The performance of the sound classifier with different binarizing thresholds is illustrated in Figure~\ref{fig:acc_vs_thr_sp}. It can be seen that the best performance for the speech is in fact obtained around the unbiased threshold of 0.5. However, for the \textit{else} class, the performance consistently decreases with the increasing threshold. This can be explained with the fact that \textit{else} class is defined rather vaguely, and the DNN probability outputs for this class are often rather small and less confident in order to avoid false detections.  

%\begin{figure}
%    \centering
%    \includegraphics[width=0.6\linewidth]{figs/detection/acc_vs_thr_sp.eps}
%    \caption{F1 score vs. binarizing threshold. Speech and direction classifier %from two separate experiments. Direction classifier assumes speech classifier works 100\% correct.}
%    \label{fig:acc_vs_thr_sp}
%\end{figure}

% \subsubsection{Performance vs. Model size}
% While implementing a real-life sound event classifier, performance is often not the only factor that needs to be considered. Computational requirements, especially for mobile devices with smaller memory, can also play an important role in selecting the optimal architecture. 

% The performance of the different size CRNN architectures based on the grid search experiments are visualized in Figure~\ref{fig:acc_vs_model_size}. One can notice that it is possible to get quite good speech classification F1 score even with the smaller models. The difference between the performances of the similar sized model highlights the importance of conducting a grid search to determine the optimal network depth and the number of units at each layer.  

% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\linewidth]{figs/detection/acc_vs_model_size.eps}
%     \caption{Speech F1 score vs. model size. The model size is determined by the number of parameters in the model.}
%     \label{fig:acc_vs_model_size}
% \end{figure}

==> Two-Stage-Hierachical (arxiv)/results_joint.tex <==


The performance for the joint sound classification and direction detection system is presented in Table~\ref{table:joint}. In the hierarchical approach, the speaker direction is estimated only when there is speech detected by the sound classifier. For frames without speech detection, the  "Speech front" and "Speech back" labels are set to zero.

The proposed hierarchical classifier has the highest performance in terms of the F1-score for the labels "Speech back" and "Something else". In contrast, the "Speech front" is overall better detected with the flat model. This is most likely attributed to the observed  difficulty in detecting the presumably more distant and thus weaker speech signals in front of the array. Since the hierarchical system only passes the frames labeled as speech, the performance is deteriorated by the errors accumulating from the two separate classification steps. The "Speech back" detection capability for the hierarchical model is significantly higher (7.5~\% points  higher in terms of F1-score) than that of the baseline, rendering the performance of the hierarchical model better in terms of overall performance. This is also evident in the unweighted average performance values, which are all higher for the proposed model in contrast to the baseline. 

%While detecting the front speaker, the flat approach has higher performance. 

%There are several factors that need to be considered while evaluating the joint system. Firstly, it should be noted that we can solely evaluate the speaker direction estimation performance only by assuming that the sound classifier performs with a 100\% precision and recall, which is the case in the panel (a) for the Table~\ref{table:joint}. On the other hand, referring to Table~\ref{table:clsf_overall}, the recall for speech classification is 87.4\%, meaning that there is a small portion of speech samples that have not been passed to speaker direction detection, so the evaluation of those samples is absent in panels (b) and (c) for Table~\ref{table:joint}, respectively. In addition, the precision for the speech classification is 89.3\%, and this affects the evaluation of the speaker direction estimation in the following way. Since the latter system is trained only using the samples with a speaker involved, there are no training samples that are not labeled either with back, front or both. However, with the joint system, the speaker direction estimator will be fed some samples which do not include speech, due to the non-100\% precision of the speech classifier. For these samples, the target direction is set as empty, which is a case not encountered during the training of the speaker direction estimator. Almost all of these samples result with an error in the direction estimation. Therefore, the panel (c) for the Table~\ref{table:joint} is helpful in interpreting the case in which the speech classifier works correctly (100\% F1 score for this subset of samples), and how much the direction estimation performance can be improved solely through the direction estimator. % \textit{AE: please check the previous sentence, cannot understand.}  

% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c|c}
%     & Precision & Recall & F1 \\
%     \toprule
%         Back &  66.6& 96.0& 78.6\\
%         Front & 96.7& 79.2& 87.1 \\
%     \end{tabular}
%     \caption{Speaker direction detection performance assuming the speech classifier works \%100 correct.}
%     \label{table:joint1}
% \end{table}
% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c|c}
%     & Precision & Recall & F1 \\
%     \toprule
%         Back &  61.0& 96.4& 74.7\\
%         Front & 82.4& 80.7& 81.5 \\
%     \end{tabular}
%     \caption{Speaker direction detection performance for the samples where sound classifier detects speech presence.}
%     \label{table:joint2}
% \end{table}

% \begin{table}
%     \centering
%     \begin{tabular}{c|c|c|c}
%     & Precision & Recall & F1 \\
%     \toprule
%         Back &  69.8& 96.4& 81.0\\
%         Front & 97.5& 80.7& 88.3 \\
%     \end{tabular}
%     \caption{Speaker direction detection performance for the samples where speech classifier \textit{correctly} detects speech presence.}
%     \label{table:joint3}
% \end{table}

% An easy-to-use way of visualizing the joint system results is the \textit{sed\_vis} toolbox~\footnote{https://github.com/TUT-ARG/sed\_vis}, written by Toni Heittola from our research group. The script to produce the necessary text files for sed\_vis can produced with\newline \texttt{cd analysis; python labels\_to\_sed\_vis.py}. \newline
% An example illustration of the sed\_vis output is given in Figure~\ref{fig:sed_vis_example}. It is also possible to follow the labels and outputs in time through an indicator bar. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figs/classification/sed_vis_example.png}
%     \caption{Visualization example for the joint system outputs.}
%     \label{fig:sed_vis_example}
% \end{figure}

==> Two-Stage-Hierachical (arxiv)/sloc.tex <==
 %\hl{Should this paragraph go to localization?}
 %The received microphone signal is a noisy mixture of source signals, each convolved with a \ac{RIR} $H_{i,n}\tfp$ between the $i$th microphone position and the $n$th source position. In the \ac{STFT} domain, the signal model can be written as
%\begin{equation}\vspace{-1mm}
%  \textstyle  X_i\tfp = \sum_n H_{i,n}\tfp S_n\tfp +  N_i\tfp,
%\end{equation}
%where $N_i\tfp$ is a mixture of interference sources, and additive noise that is independent between microphones, and $\omega_k=\jmath 2\pi k/K$ is the angular frequency with $K$ discrete DFT bins. 
%\hl{Maybe mention we combine front-left, front and front-right as "front" (and same for "back") due to practical reasons (low amount of data)}

The task of the localization step is to assign the labels of "Speech front" and "Speech back" to each 1-s block of audio, detected to contain speech in the first stage. %Refer to Fig.~\ref{fig:array} for an illustration of the array geometry and sound direction labels.
%
%The time sequence of directional labels of "speech front" and "speech back" is not assumed to be significant during the one second audio block, and only the appearance of either or both directions within the block is of interest. Therefore, 
%
%
%The CRNN architecture is  also used to solve the direction classification task by mapping a sequence of feature vectors into output probabilities or direction labels. % and processes them to output a two dimensional vector $\mathbf{o}=[o_1,o_2]^\textnormal{T}$ with values $o_i \in [0,1]$.
%
%The model architecture selected here is a , and the input is a set of concatenated feature values corresponding to one second input signal. %For a description of a \ac{CNN}, refer to e.g. \cite{chollet}.  The features with default parameter values include the pairwise \ac{TDOA} from channels (1,3) and (2,4), and they are of dimension $F \times P$, where $P=2$ is the number of pairs. The $F \times B$ magnitude features are obtained by averaging the magnitude differences of the same pairs. In total, there are $F\times (B+P)$ feature values per one second. 
%
 % The structure of the \ac{CNN} is listed in Table~\ref{table:cnn1}, and it %
 %
% 
%The magnitude spectrum features for the speech and "something else" classifier do not include spatial information about the speech source. However, s
%
% Spatial information about the source is required to classify its direction.
The speaker direction is assumed to be more stable compared to changes in the magnitude spectrum, and therefore longer 85~ms frames with 50~\% overlap are utilized. Two types of spatial features are extracted.

\ssection{\ac{TDOA} Feature}
The \ac{TDOA}, i.e. the sound propagation delay between a microphone pair, brings information about the dominating sound direction during each short processing frame. The case with speakers in front and back is evident by alternating \ac{TDOA} values. % between the speakers during the one-second block. 

%Since the task is to locate speech in front and/or back of the array, the microphone pairs that are maximally separated in this axis produce the most spatial information. 
 %
%They were estimated separately between two microphone pairs that had one of the microphones in the front and the other in the back surface of the device, and otherwise in the same (x,y) position, refer to Fig.~\ref{fig:array}.
%
%Therefore, two microphone pairs (1,3) and (2,4) located on the front and back surfaces on the left and right side of the device were used for TDOA estimation and are displayed in Fig.~\ref{fig:array}. 


 %
%The parameters (window length, amount of overlap, and window shape) of the feature extraction are defined in the \texttt{parameters} struct, and their values are illustrated in Table~\ref{table:defaultvalues}. The default window lenght is 4096 samples.
 %
% \hl{The default values are pairs (1,3) and (2,4), which correspond to forward and backward facing microphone pairs in the left and right side of the mobile array.%, refer to Fig~\ref{fig:arraygeometry}.
% 
 %
Since the microphone pair separation in the front-back axis is only 7~mm, the \ac{TDOA} resolution is limited to three possible values at 48~kHz. Therefore, \ac{TDOA} is obtained as maximum peak index of Fourier interpolated (factor of five) \ac{GCC}~\cite{Knapp:1976:TASLP} between microphones. 
%\begin{eqnarray}\label{eq:srp}\vspace{-2mm}
%\gcc{}{ij} = 
%\textstyle 
% { \sum_{k=0}^{K-1} } \frac{ \mic{i}{} \!\cdot\!  \mic{j}{{\ast}}\!   } { \arrowvert \mic{i}{} \arrowvert \!\!\cdot\!\! \arrowvert \mic{j}{\ast} \arrowvert }  e^{\jmath \cdot \tau \cdot \omega_k},vspace{-2mm}
%\end{eqnarray}
% is used as the \ac{TDOA}%, where $(\cdot)^\ast$ denotes complex conjugate, and $\tau$ is a \ac{TDOA}
%The two \ac{TDOA} values are averaged over the microphone pairs for robustness and to reduce the \ac{TDOA} feature dimension to one.
 %However, the microphone  separation in the front-back axis is only 7~mm, which means that all observed \ac{TDOA} values are between $[-1,+1]$ samples at 48~kHz sampling rate. Therefore, sub-sample Fourier interpolation with a factor of five is used to obtain more detailed \ac{TDOA} values.  
 
%The 7~mm microphone pair separation results in \ac{TDOA} values between $[-1,+1]$ samples at 48~kHz sampling rate, and threfore five-time sub-sample Fourier interpolation is used to obtain higher  \ac{TDOA} resolution. 
 
 %The estimate for \ac{TDOA}  between a single microphone pair is then obtained at time fram
 
 
 %e $t$%
%\begin{equation}\vspace{-1mm}%
%\label{eq:doapoint}%
%\hat{\tau}_{ij} = \argmax_{\tau} \gcc{}{ij}.\vspace{-1mm}%
%\end{equation}%
%The interpolation is done by calculating $\tau$ in \eqref{eq:srp} with $I$ interpolated delay values for each sample delay. Default values are $T=15$ (48kHz) and $I=5$, and $I=1$ would omit the interpolation. 

%Figure~\ref{fig:tdoa} illustrates the feature behavior for a 10 s white noise sound source directly in front of the array in panel a) and front camera view is displayed in panel c). The default microphone pairs (see Table \ref{table:defaultvalues} are used. Note that their value is negative and similar to each other. In panel b) the sound source is in the back side of the device, and the corresponding features are now of the opposite sign. This demonstrates that the features correspond to the physical location of the sound source.

%The peak-picking method of Eq~\eqref{eq:doapoint} allows to capture a situation with sound in the front and back of the array if the sounds sources alternate in time-frequency domain and therefore cause the \ac{TDOA} estimate to switch between sources. To further allow evidence from two spatially separate sound sources, the direct GCC vector can be considered from \eqref{eq:srp} as $\gcc{}{ij}$. 


%\begin{figure}[!t]
%	\centering
%	\includegraphics[width=.7\columnwidth]{report/figs/Slide1a.png}
%	\caption{The magnitude difference features for a loudspeaker playing white Gaussian noise, refer to Fig.~\ref{fig:tdoa}.}
%	\label{fig:magdiff}
%\end{figure}
%
\ssection{Magnitude Difference Feature}
Upon reaching the rigid device, the sound wave is partly reflected and partly diffracted, leading to frequency and angle dependent sound propagation effects. This is observed as a direction specific level difference between the microphones.
 %
% The attenuation of a sound wave reaching the microphones depends on the inclination angle and the dimensions of the mobile device with respect to each wavelength due to acoustic shadowing. 
% 
 The magnitude difference between the microphone pairs is used as the second spatial feature to capture this information: % It is defined and its values are illustrated in this subsection. 
%
%\begin{equation}
 $   D_{i,j}(b) =  \ln (M_i(b)) - \ln (M_j(b))$,
%\end{equation}
where $M_i(b)$ is the % mel-frequency resolution magnitude spectrum and $b$ refers to the $b$th mel-frequency band. The total number of used mel-bands is $40$. The feature value was similarly averaged over the pairs. 
  magnitude of the $b$th mel band of microphone $i$. The total number of  mel-bands was $40$. %The feature values are also % similarly obtained from and
%  averaged over the two microphone pairs (1,3) and (2,4). 


Features are obtained from two microphone pairs (1,3) and (2,4) located on the front and back surfaces on the left and right side of the device. The pairs are maximally separated in the dimension of interest, refer to Fig.~\ref{fig:array}. Both features are then averaged over the microphone pairs for robustness and to reduce the feature dimension by half.

 \paragraph*{\ac{DNN} Model for Localization}
As for sound event detection, the used model was a CRNN, where now two output values are related to  probabilities of speech front, and speech back. A similar training process and validation method was used as in Section~\ref{subsec:speechtrain}. %, except that three folds were used for training, two for validation, and one for testing. This is due to lack of directional diversity in a single validation set. Also, 
  %, which consisted of four convolution layers with \ac{ReLU} activation functions. Each convolution was followed by max pooling operation to reduce both the temporal and the feature dimensions. The last pooling layer reduces the feature dimension and the time dimension to one, and all the information is encoded into the feature maps. The collapsing of the time-dimension is motivated by making the model invariant to the temporal location of the events. Three fully connected layers with \ac{ReLU} activation functions are then stacked after the last max pool layer. The convolution layers and the fully connected layers share a common $\ell_2$-regularization value, which results in the scaled increase of the objective function value with the $\ell_2$-norm of the weights~\cite{Haykin:1999}. These layers are followed by a dropout layer~\cite{srivastava2014dropout}, that is finally connected to the output layer with sigmoid -type activation functions. 
%
% obtained by multiplying the $i$th microphone signal's magnitude spectrum $|X_i\tfp|$ with a weight matrix $W(\omega_k,b)$ that defines a mel-filterbank, consisting of equally spaced triangular filters overlapping with adjacent bands (refer e.g. to~\cite{woelfel2009distant}), and $b$ refers to the $b$th mel-frequency band. The total number of used mel-bands is $40$. % (default value 40). 
%
%
%
%Figure~\ref{fig:magdiff} illustrates the feature behavior for a 10 s recording of white noise, using the default microphone pairs (see Table \ref{table:defaultvalues}). Note that the magnitude difference is small in the first 15 mel bands when the signal starts at 2s mark. In the upper frequency range, the feature has non-zero values. This is most likely due to shadowing effect of sound propagation, where objects smaller than the wavelength do not interfere with the wavefront. Similarly, wavelengths that are smaller than the object shape will reflect from the surface. Unlike the \ac{TDOA} feature, the feature value is evaluated for each frequency band separately.
%
%
%
%
%\subsubsubsection{Feature Scaling}
%The real data is divided into six folds, and processed with k-fold-cross validation. Three folds are used for training, two for validation, and one for testing.
%The input features are scaled by setting them to zero mean (by removing the mean estimate) and having a standard deviation of one (by dividing with the standard deviation estimate). The mean and standard deviation values are estimated from the training data. They are then applied to the training, validation, and test data.
% 
% A similar approach to feature scaling as in the Section~\ref{sec:speech} was applied.
 %
%\subsubsubsection{Training Procedure}
%The training loops over different types of hyper-parameters, including the number of neurons $N_n$, number of filters $N_c$, dropout probability $p$, batch size, L2-regularization, convolution kernel dimension. 
 %
%The training minimized the binary cross-entropy between the ground truth label and the predicted output. The training was done in mini-batches.  The number of neurons in the fully connected layers, the number of convolution filters in the \ac{CNN}, optimizer type, dropout rate, $\ell_2$-regularization, and dimensions of the \ac{CNN} kernel were selected via a grid search using validation data. %The optimization algorithm minimizes the cost function.
The Adam and Adamax~\cite{Kingma:ICLR:2015} %and adagrad~\cite{adagrad}
 optimizers were experimented with.
 %
%function grows near 0. Also, in the page \pageref{fig:frontback} 
 %
%\subsubsubsection{Training with Real Data}
%The section~\ref{sec:realdatacollection} describes the real-data collection method. This section describes, how the real-data was used to train the front/back classifier.
%
%
The training was done using k-fold-cross-validation with all one-second blocks containing speech from the folds listed in Table~\ref{tab:classdir}. Three of the folds were used for training, two for validation, and one for testing to guarantee sufficient number of directional labels in the validation set. % The table represents the multilabel information of the two classes using a categorical split into three separate classes, where the class "both" represents the number of blocks where "speech front" and "speech back" are simultaneously active, and "speech front" and "speech back" indicate the number of blocks  where only either label is present. 
%
 %The validation set was used to stop the training process by monitoring the decrease of the validation set's average F1-score over both direction labels. 
  The training was stopped if validation set's average F1-score over both direction labels started to decrease. 
 %
Note that the case where both "Speech front" and "Speech back" are active is underrepresented, with only 6~\% of the samples belonging to this class. As a consequence, the speech samples are labeled as either with "Speech back" or "Speech front" labels, and the cases where both labels are active is effectively ignored. To address this data imbalance, a random oversampling strategy~\cite{VanHulse:2007} was applied to balance training and validation sets during training so that each unique combination of label values (i.e. class) would have the same amount of (partly repeated) training sequences. This reduced slightly the final F1-score in contrast to not using oversampling, but raised the performance of detecting speech in both directions. %Without considering the class imbalance, the network tries to propose a trivial solution, where
 %While this results in a good overall F1-score, it does not actually recognize simultaneous speech in front and back directions. 
 %
The best model had 170k parameters. 

==> Two-Stage-Hierachical (arxiv)/tabledata.tex <==

\ifoldr

\addtolength{\tabcolsep}{-4.5pt} 
%
\begin{table}[!b]
\vspace{-4mm}
    \centering \caption{Amount of recorded seconds for each environment type.}
    \label{tab:environments}\vspace{-2.3mm}
    \scalebox{0.65}{
    \begin{tabular}{ |c| c| c| c| c| c| c| c| c| c| c| c| c| c| c| c| c| c| c| c| c| c| c| c|  }
         \hline
        \rotatebox{90}{Apartment} &
        \rotatebox{90}{Industrial area} &
        \rotatebox{90}{Club room} &
        \rotatebox{90}{Studio room} 
        &\rotatebox{90}{Street} 
        &\rotatebox{90}{Meeting room} 
        &\rotatebox{90}{Corridor/office } &
        \rotatebox{90}{Park} &
        \rotatebox{90}{Live club} &
        \rotatebox{90}{Car} &
        \rotatebox{90}{Urban area} &
        \rotatebox{90}{Stairs} &
        \rotatebox{90}{Lake} &
        \rotatebox{90}{Cycle path} &
        \rotatebox{90}{Ship's deck} &
        \rotatebox{90}{Subway} &
        \rotatebox{90}{Store room} &
        \rotatebox{90}{Grocery store} &
        \rotatebox{90}{Marketplace} &
        \rotatebox{90}{Beach} &
        \rotatebox{90}{Harbour} & 
        \rotatebox{90}{Terrace} &
        \rotatebox{90}{Cafe} & 
        \rotatebox{90}{Terminal} \\
        \hline
           \rotatebox{90}{1094 }&
           \rotatebox{90}{920}&
           \rotatebox{90}{630}& 
           \rotatebox{90}{419}&
           \rotatebox{90}{404}&
           \rotatebox{90}{335}&
           \rotatebox{90}{245}&
           \rotatebox{90}{226}& 
           \rotatebox{90}{210}&
           \rotatebox{90}{185}&
           \rotatebox{90}{110}&
           \rotatebox{90}{105}& 
           \rotatebox{90}{65}&
           \rotatebox{90}{60}&
           \rotatebox{90}{60}& 
           \rotatebox{90}{51}& 
           \rotatebox{90}{45}&
           \rotatebox{90}{41}& 
           \rotatebox{90}{40}&
           \rotatebox{90}{20}&
           \rotatebox{90}{20}&
           \rotatebox{90}{15}& 
           \rotatebox{90}{15}& 
           \rotatebox{90}{11}\\
           \hline
    \end{tabular}
    } %\vspace{-4mm}
\end{table}
\addtolength{\tabcolsep}{4.5pt} 


\fi



\addtolength{\tabcolsep}{-1pt} 
%
\begin{table}[!b]
\vspace{-4mm}
    \centering
        \caption{Duration (s) of recordings for each environment.}
    \label{tab:environments}\vspace{-2.3mm}
    \scalebox{0.8}{
    \begin{tabular}{ |l c| l c| l c|l c |    }
         \hline
        {Apartment} & 1094 &
       {Industrial area} & 920 &
        {Club room} & 630 &
        {Studio room}& 419  \\ \hline
        {Street} & 404 & 
        {Meeting room} & 335 &
        {Corridor/office} & 245 &
        {Park} &226 \\ \hline
        {Live club} &210 & 
        {Car} &185 &
        {Urban area} &110 &
        {Stairs} &105 \\ \hline
        {Lake} &65  & 
        {Cycle path} &60 &
        {Ship's deck} &60 &
        {Subway} &51 \\ \hline
        {Store room} &45 & 
        {Grocery store} &41 & 
        {Marketplace} &40 &
        {Beach} &20 \\ \hline
        {Harbour} & 20 & 
        {Terrace} &15 &
        {Cafe} & 15 &
        {Terminal} & 11 \\
           \hline
    \end{tabular}
    } %\vspace{-4mm}
\end{table}
\addtolength{\tabcolsep}{1pt} 




==> Two-Stage-Hierachical (arxiv)/tabledetection.tex <==

\ifoldr
\begin{table}[b] 
\vspace{-5mm}
    \caption{Overall performance of the proposed CRNN method for sound classification.}
    \label{table:clsf_overall} 
    \centering\scalebox{1}{
    \begin{tabular}{c|c|c|c}
    & Precision & Recall & F1 (\%) \\
    \toprule
        Speech (Back or Front) &  89.3& 87.4& 88.4\\
        Something else & 76.6& 63.9& 69.7 \\
    \end{tabular}} 
%
%
\end{table}
\fi


\ifnewr\ifoldr
\begin{table}[b] 
\vspace{-5mm}
    \caption{Performance of the hirearchical CRNN method for sound classification.}
    \label{table:clsf_overall} 
    \centering\scalebox{1}{
    \begin{tabular}{c|c|c|c}
    & Precision & Recall & F1 (\%) \\
    \toprule
% Speech precision, recall, F1 score at thr 0.5: 0.8777, 0.8983, 0.8879
% Something else precision, recall, F1 score at thr 0.5: 0.7504, 0.6134, 0.6750

        Speech (Back or Front) &  87.8& 89.8& 88.8\\
        Something else & 75.0 & 61.3& 67.5 \\
    \end{tabular}} 
%
%Speech precision, recall, F1 score at thr 0.1: 0.7373, 0.9542, 0.8318
% Something else precision, recall, F1 score at thr 0.1: 0.5079, 0.7908, 0.6186
%
%Speech precision, recall, F1 score at thr 0.2: 0.7966, 0.9300, 0.8581
%Something else precision, recall, F1 score at thr 0.2: 0.5782, 0.7251, 0.6434
%
%Speech precision, recall, F1 score at thr 0.3: 0.8252, 0.9126, 0.8667
%Something else precision, recall, F1 score at thr 0.3: 0.6209, 0.6693, 0.6442
%
%Speech precision, recall, F1 score at thr 0.4: 0.8471, 0.8967, 0.8712
%Something else precision, recall, F1 score at thr 0.4: 0.6593, 0.6212, 0.6397
%
%Speech precision, recall, F1 score at thr 0.5: 0.8614, 0.8793, 0.8703
%Something else precision, recall, F1 score at thr 0.5: 0.6861, 0.5822, 0.6299
%
%Speech precision, recall, F1 score at thr 0.6: 0.8784, 0.8582, 0.8682
%Something else precision, recall, F1 score at thr 0.6: 0.7129, 0.5374, 0.6128%
%
%Speech precision, recall, F1 score at thr 0.7: 0.8910, 0.8351, 0.8622
%Something else precision, recall, F1 score at thr 0.7: 0.7359, 0.4925, 0.5901%
%
%Speech precision, recall, F1 score at thr 0.8: 0.9120, 0.7961, 0.8502
%Something else precision, recall, F1 score at thr 0.8: 0.7617, 0.4444, 0.5613
%
%Speech precision, recall, F1 score at thr 0.9: 0.9390, 0.7160, 0.8124
%Something else precision, recall, F1 score at thr 0.9: 0.7975, 0.3736, 0.5088
%
%
%Final F1 score = 0.870297585626.
%%Confusion matrix, without normalization
%[[1030  167  190   41] silence
% [ 208 1669   29  150] speech
% [ 326  120  459   46] else
% [  25  172   57  334]] both
%Normalized confusion matrix
%[[0.72128852 0.11694678 0.13305322 0.02871148]
% [0.10116732 0.81177043 0.01410506 0.0729572 ]
% [0.34279706 0.12618297 0.48264984 0.04837014]
% [0.04251701 0.29251701 0.09693878 0.56802721]]


\end{table}

% Speech front precision, recall, F1 score at thr 0.5: 0.8702, 0.8877, 0.8788
% Speech back precision, recall, F1 score at thr 0.5: 0.7204, 0.7801, 0.7491
% Something else precision, recall, F1 score at thr 0.5: 0.7110, 0.6075, 0.6552


\fi\fi


\ifoldr

\addtolength{\tabcolsep}{-2pt} 
\begin{table}[t]
\caption{Confusion matrix of the proposed \ac{CRNN} method for sound detection. The instances where both classes are present are treated as a separate class for the visualization.}
    \label{fig:clsf_overall} 
\newcommand\items{4}   %Number of classes
\arrayrulecolor{white} %Table line colors
\noindent
\scalebox{0.9125}{
\begin{tabular}{cc*{\items}{|c}|}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{\items}{c}{Predicted label} \\ \hhline{~*\items{|-}|}
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{\rot{Nothing}} & 
\multicolumn{1}{c}{\rot{Speech}} & 
\multicolumn{1}{c}{\rot{Else}} &
\multicolumn{1}{c}{\rot{Both}} \\ \hhline{~*\items{|-}|}
\multirow{\items}{*}{\rotatebox{90}{Actual label}} 
&Nothing  & 1114   & 140  & 164 & 10   \\ \hhline{~*\items{|-}|}
&Speech  & 203   & 1727  & 18 & 108   \\ \hhline{~*\items{|-}|}
&Else  & 302   & 76   & 523 & 50\\ \hhline{~*\items{|-}|}
&Both  & 35   & 143   & 76 & 334 \\ \hhline{~*\items{|-}|}
\end{tabular}%
}\hspace{-4mm}%
\renewcommand\items{4}   %Number of classes
\arrayrulecolor{white} %Table line colors
\noindent
\scalebox{0.9125}{
\begin{tabular}{cc*{\items}{|E}|}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{\items}{c}{Predicted label} \\ \hhline{~*\items{|-}|}
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{\rot{Nothing}} & 
\multicolumn{1}{c}{\rot{Speech}} & 
\multicolumn{1}{c}{\rot{Else}} &
\multicolumn{1}{c}{\rot{Both}} \\ \hhline{~*\items{|-}|}
\multirow{\items}{*}{\rotatebox{90}{ }} 
&Nothing & 78.0& 9.8& 11.5& 0.7 \\ \hhline{~*\items{|-}|} 
&Speech  &  9.9& 84.0& 0.9& 5.3 \\ \hhline{~*\items{|-}|} 
&Else  &31.8& 8.0& 55.0& 5.3 \\ \hhline{~*\items{|-}|} 
&Both  & 6.0& 24.3& 12.9& 56.8 \\ \hhline{~*\items{|-}|} 
\end{tabular}
}
\addtolength{\tabcolsep}{2pt} 
\vspace{-5mm}
\end{table}

\fi



\ifnewr

\addtolength{\tabcolsep}{-3pt} 
\begin{table}[t]\vspace{-0mm}
\caption{The confusion matrix of SED (proposed).}
%\caption{The confusion matrix of the proposed hierarchical \ac{CRNN} method for speech and else class detection. } % The instances where both classes are present are treated as a separate class for the visualization.}
    \label{fig:clsf_overall} \vspace{-2mm}
\newcommand\items{4}   %Number of classes
\arrayrulecolor{white} %Table line colors
\noindent
\scalebox{0.895}{
\begin{tabular}{cc*{\items}{|c}|}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{\items}{c}{Predicted label} \\ \hhline{~*\items{|-}|}
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{[frames]} & 
\multicolumn{1}{c}{{Nothing}} & 
\multicolumn{1}{c}{{Speech}} & 
\multicolumn{1}{c}{{Else}} &
\multicolumn{1}{c}{{Both}} \\ \hhline{~*\items{|-}|}
\multirow{\items}{*}{\rotatebox{90}{True label}} 
% model 143 
% Normalized confusion matrix
% [[0.76890756 0.1092437  0.11344538 0.00840336]
% [0.08706226 0.84484436 0.00680934 0.06128405]
% [0.33964248 0.11041009 0.48895899 0.06098843]
% [0.04761905 0.23639456 0.08163265 0.63435374]]
% 2020-01-27 02:30:25.818117
&Nothing  & \bf1098   & 156  & 162 & 12   \\ \hhline{~*\items{|-}|}
&Speech  &179 & \bf1737 &  14 & 126   \\ \hhline{~*\items{|-}|}
&Else  & 323 & 105 & 465  & 58 \\ \hhline{~*\items{|-}|}
&Both  &28 & 139 & 48 & \bf373\\ \hhline{~*\items{|-}|}
\end{tabular}%
}\hspace{-4mm}%
\renewcommand\items{4}   %Number of classes
\arrayrulecolor{white} %Table line colors 
\noindent
\scalebox{0.9}{
\begin{tabular}{cc*{\items}{|E}|}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{\items}{c}{Predicted label} \\ \hhline{~*\items{|-}|}
\multicolumn{1}{c}{} & 
\multicolumn{1}{l}{[\%]} & 
\multicolumn{1}{c}{\hspace{-5.5mm}{Nothing}} & 
\multicolumn{1}{c}{\hspace{-3.3 mm}{~Speech}} & 
\multicolumn{1}{c}{\hspace{-2 mm}{Else}} &
\multicolumn{1}{c}{{Both}} \\ \hhline{~*\items{|-}|}
\multirow{\items}{*}{\rotatebox{90}{ }} 
&Nothing & 76.9  & 10.9 &  11.3  &  0.8 \\ \hhline{~*\items{|-}|} 
&Speech  &  8.7  & 84.5 &   0.7  &  6.1  \\ \hhline{~*\items{|-}|} 
 &Else   &  34.0 & 11.0 &  48.9  &  6.1 \\ \hhline{~*\items{|-}|} 
&Both    &  4.8  & 23.6 &   8.2  & 63.4  \\ \hhline{~*\items{|-}|} 
\end{tabular}
}
\vspace{-3mm}
\end{table}
\addtolength{\tabcolsep}{3pt} 

\fi





%%%%%%%%%%%% BASELINE %%%%%%%%%%%%%%%%%
\ifnewr

\addtolength{\tabcolsep}{-3pt} 
\begin{table}[t]
\caption{The confusion matrix of SED (baseline).}
%\caption{The confusion matrix of the flat baseline \ac{CRNN} method for (merged) speech and else class detection.}% The instances where both classes are present are treated as a separate class for the visualization.}
    \label{fig:clsf_overall_baseline} \vspace{-2mm}
\newcommand\items{4}   %Number of classes
\arrayrulecolor{white} %Table line colors
\noindent
\scalebox{0.9}{
\centering
\begin{tabular}{cc*{\items}{|c}|}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{\items}{c}{Predicted label} \\ \hhline{~*\items{|-}|}
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{[frames]} & 
\multicolumn{1}{c}{{Nothing}} & 
\multicolumn{1}{c}{{Speech}} & 
\multicolumn{1}{c}{{Else}} &
\multicolumn{1}{c}{{Both}} \\ \hhline{~*\items{|-}|}
\multirow{\items}{*}{\rotatebox{90}{~True label}} 
&Nothing  & 1037 & 194 & 173 &  24   \\ \hhline{~*\items{|-}|}
&Speech  &266 &1575 &  38 & 177   \\ \hhline{~*\items{|-}|}
&Else  &210 & 152& \bf 511 &  78 \\ \hhline{~*\items{|-}|}
&Both  &40 & 166 & 104 & 278\\ \hhline{~*\items{|-}|}
\end{tabular}%
}\hspace{-4mm}%
\renewcommand\items{4}   %Number of classes
\arrayrulecolor{white} %Table line colors 
\noindent
\scalebox{0.89}{
\begin{tabular}{cc*{\items}{|E}|}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{\items}{c}{Predicted label} \\ \hhline{~*\items{|-}|}
\multicolumn{1}{c}{} & 
\multicolumn{1}{l}{[\%]} & 
\multicolumn{1}{c}{\hspace{-5.5mm}{Nothing}} & 
\multicolumn{1}{c}{\hspace{-3.3 mm}{~Speech}} & 
\multicolumn{1}{c}{\hspace{-2 mm}{Else}} &
\multicolumn{1}{c}{{Both}} \\ \hhline{~*\items{|-}|}
\multirow{\items}{*}{\rotatebox{90}{ }} 
&Nothing &  72.6 &  13.6 &  12.1 &   1.7 \\ \hhline{~*\items{|-}|} 
&Speech  &  12.9 & 76.6  &  1.8  &  8.6 \\ \hhline{~*\items{|-}|} 
 &Else   &  22.1 &  16.0 & 53.7 &   8.2 \\ \hhline{~*\items{|-}|} 
&Both    &  6.8 &  28.2 &  17.7 &  47.3 \\ \hhline{~*\items{|-}|} 
\end{tabular}
}
\vspace{-6mm}
\end{table}
\addtolength{\tabcolsep}{3pt} 

\fi


==> Two-Stage-Hierachical (arxiv)/tablejoint.tex <==

\ifoldr
\arrayrulecolor{black} %Table line colors
\addtolength{\tabcolsep}{-2pt} 
\begin{table}[hb]
\vspace{-5mm}
    \centering
    \caption{Speaker direction detection performance (a): assuming the speech classifier works \%100 correct, (b): for the samples where sound classifier detects speech presence, (c): for the samples where speech classifier \textit{correctly} detects speech presence.}
    \label{table:joint}    
    \scalebox{1}{
\begin{tabular}{cc|c|c|c}
    &  & Precision & Recall & F1 \\
    \toprule
     (a) & Front   &  87.3& 95.7& 91.3\\
      & Back  & 91.5& 96.1& 93.7 \\
    \midrule
     (b)&  Front  &  83.9& 97.3& 90.1\\
      &  Back & 79.6& 95.8& 86.9 \\
\midrule
     (c) &  Front  &  89.6& 97.3& 93.3\\
       & Back   & 91.7& 95.8& 93.7 \\
    \end{tabular}
    } 
\end{table}
\addtolength{\tabcolsep}{2pt} 
\fi

\ifnewr
\arrayrulecolor{black} %Table line colors
\addtolength{\tabcolsep}{-3pt} 
\begin{table}[t]
\vspace{-0mm}
    \centering
    \caption{Speaker direction and else class detection performance (A): proposed hierarchical approach, (B): baseline  }\vspace{-2mm}
    \label{table:joint}    
    \scalebox{1}{
\vspace{-1mm}
\scalebox{0.9}{
\begin{tabular}{cc|c|c|c|c}
    & Label & Accuracy \%& Precision \%& Recall \%& F1 \%\\
    \toprule
%Speech front precision, recall, F1 score at thr 0.5: 0.8432, 0.8957, 0.8687
%Speech back precision, recall, F1 score at thr 0.5: 0.7932, 0.8436, 0.8177
%Else precision, recall, F1 score at thr 0.5: 0.7504, 0.6134, 0.6750
%Accuracy score for speech front 0.952219788971, speech back 0.852478598447, else 0.819032450727

     (A) & Speech front  & 95.2 &  84.3& \bf 89.6& 86.9\\
      & Speech back  & \bf 85.2 &\bf 79.3& \bf 84.4& \bf 82.8 \\
      & Something else & \bf 81.9 & \bf 75.0& 61.3& \bf 67.5 \\
    %\midrule
    & Average (unweighted) & \bf 87.4 & \bf 79.5 & \bf 78.4 & \bf 79.1 \\
    \midrule
%Speech front precision, recall, F1 score at thr 0.5: 0.9234, 0.8706, 0.8962
%Speech back precision, recall, F1 score at thr 0.5: 0.7583, 0.7486, 0.7534
%Something else precision, recall, F1 score at thr 0.5: 0.7021, 0.6309, 0.6646
% Accuracy score for speech front 0.959984073263, speech back 0.823412303404, else 0.80489747163

(B)&  Speech front  & \bf 96.0 & \bf 92.3 &  87.1 & \bf 89.6 \\
      &  Speech back & 82.3 &75.8 & 74.9 & 75.3 \\
      &  Something else &80.5 &70.2 & \bf 63.1 & 66.5 \\
    %\midrule
    & Average (unweighted) & 86.3 & 79.4 & 75.0 & 77.1 \\
    \end{tabular}}
    } \vspace{-6mm}
\end{table}
\addtolength{\tabcolsep}{3pt} 
\fi


==> Two-Stage-Hierachical (arxiv)/tablelocres.tex <==

\ifoldr
\addtolength{\tabcolsep}{-1pt} 
\begin{table}[t]
\caption{Confusion matrices of speech localization computed over the folds. Left table shows  accumulated results, right table shows relative results. The instances where both classes are present are treated as a separate class for the visualization.}\label{table:resdir}
\newcommand\items{3}   %Number of classes
\arrayrulecolor{white} %Table line colors
\noindent
\centering
\scalebox{1}{
\begin{tabular}{cc*{\items}{|c}|}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{\items}{c}{Predicted label} \\ \hhline{~*\items{|-}|}
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{\rot{Back}} & 
\multicolumn{1}{c}{\rot{Front}} & 
\multicolumn{1}{c}{\rot{Both}} \\ \hhline{~*\items{|-}|}
\multirow[t]{\items}{*}{\rotatebox{90}{\hskip -25pt Actual label}} 
&Back  & 1508   & 18  & 121   \\ \hhline{~*\items{|-}|}
&Front  & 21   & 672  & 141   \\ \hhline{~*\items{|-}|}
&Both  & 22   & 52   & 89  \\ \hhline{~*\items{|-}|}
\end{tabular}%
}
%\hspace{2cm}%
\arrayrulecolor{white} %Table line colors
\noindent
\scalebox{1}{
\begin{tabular}{cc*{\items}{|E}|}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{\items}{c}{Predicted label} \\ \hhline{~*\items{|-}|}
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{\rot{Back}} & 
\multicolumn{1}{c}{\rot{Front}} & 
\multicolumn{1}{c}{\rot{Both}} \\ \hhline{~*\items{|-}|}
&Back  & 91.6   & 1.1  & 7.3   \\ \hhline{~*\items{|-}|}
&Front  & 2.5   & 80.6  & 16.9   \\ \hhline{~*\items{|-}|}
&Both  & 13.4   & 31.9   & 54.6  \\ \hhline{~*\items{|-}|}
\end{tabular} 
}
\vspace{-5mm}
\end{table}
\addtolength{\tabcolsep}{1pt} 

\fi




\ifnewr 
\addtolength{\tabcolsep}{-2pt} 
\begin{table}[b]\vspace{-2mm}
\caption{Speech localization confusion matrix (proposed). \label{table:resdir}}%The instances where both classes are present are treated as a separate class for the visualization.}
\vspace{-3mm}
\newcommand\items{3}   %Number of classes
\arrayrulecolor{white} %Table line colors
\noindent
\centering
\scalebox{0.90}{
\begin{tabular}{cc*{\items}{|c}|}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{\items}{c}{Predicted label} \\ \hhline{~*\items{|-}|}
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{[frames]} & 
\multicolumn{1}{c}{{Front}} & 
\multicolumn{1}{c}{{Back}} & 
\multicolumn{1}{c}{{Both}} \\ \hhline{~*\items{|-}|}
\multirow[t]{\items}{*}{\rotatebox{90}{\hskip -20pt True label}} 
&Front  & 676 & 20 &138\\ \hhline{~*\items{|-}|}
&Back  & 23     & 1558    & 66    \\ \hhline{~*\items{|-}|}
&Both  &    58 & 28     & 77   \\ \hhline{~*\items{|-}|}
\end{tabular}%
\vspace{-2mm}
}
%\hspace{2cm}%
\arrayrulecolor{white} %Table line colors
\noindent
\scalebox{.85}{
\begin{tabular}{cc*{\items}{|E}|}
\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{\items}{c}{Predicted label} \\ \hhline{~*\items{|-}|}
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{[\%]} & 
\multicolumn{1}{c}{{Front}} & 
\multicolumn{1}{c}{{Back}} & 
\multicolumn{1}{c}{{Both}} \\ \hhline{~*\items{|-}|}
&Front &  81.1  & 2.4   & 16.5    \\ \hhline{~*\items{|-}|}
&Back  &  1.4   & 94.6  & 4.0    \\ \hhline{~*\items{|-}|}
&Both  &  35.6  & 17.2  & 47.2  \\ \hhline{~*\items{|-}|}
\end{tabular} 
}
\vspace{-5mm}
\end{table}
\addtolength{\tabcolsep}{2pt} 

